The Interplay Between Physical Activity, Protein Consumption, and Sleep Quality in Muscle Protein Synthesis

This systematic review examines the synergistic and individual influences of resistance exercise, dietary protein supplementation, and sleep/recovery on muscle protein synthesis (MPS). Electronic databases such as Scopus, Google Scholar, and Web of Science were extensively used. Studies were selected based on relevance to the criteria and were ensured to be directly applicable to the objectives. Research indicates that a protein dose of 20 to 25 grams maximally stimulates MPS post-resistance training. It is observed that physically frail individuals aged 76 to 92 and middle-aged adults aged 62 to 74 have lower mixed muscle protein synthetic rates than individuals aged 20 to 32. High-whey protein and leucine-enriched supplements enhance MPS more efficiently than standard dairy products in older adults engaged in resistance programs. Similarly, protein intake before sleep boosts overnight MPS rates, which helps prevent muscle loss associated with sleep debt, exercise-induced damage, and muscle-wasting conditions like sarcopenia and cachexia. Resistance exercise is a functional intervention to achieve muscular adaptation and improve function. Future research should focus on variables such as fluctuating fitness levels, age groups, genetics, and lifestyle factors to generate more accurate and beneficial results.

==> citelist <==
[1] \cite{gordon2013regulation}
[2] \cite{wolfe2012role}
[3] \cite{atherton2012muscle}
[4] \cite{phillips2012regulation}
[5] \cite{knowles2018inadequate}
[6] \cite{kraemer2005hormonal}
[7] \cite{cassilhas2007impact}
[8] \cite{braith2008resistance}
[9] \cite{hong2018effects}
[10] \cite{koltyn1998perception}
[11] \cite{toigo2006new}
[12] \cite{strickland2014anxiolytic}
[13] \cite{kallman1990role}
[14] \cite{peterson2011resistance}
[15] \cite{melov2007resistance}
[16] \cite{storer2001exercise}
[17] \cite{evans2010skeletal}
[18] \cite{landi2019muscle}
[19] \cite{dattilo2020effects}
[20] \cite{dattilo2011sleep}
[21] \cite{lin2022effect}
[22] \cite{freitas2020sleep}
[23] \cite{saner2020effect}
[24] \cite{driver2000exercise}
[25] \cite{uchida2012exercise}
[26] \cite{vierck2000satellite}
[27] \cite{schiaffino2013mechanisms}
[28] \cite{berk2001vascular}
[29] \cite{pallafacchina2013role}
[30] \cite{tidball2005mechanical}
[31] \cite{keskin2008principles}
[32] \cite{wu2016dietary}
[33] \cite{westerterp2009dietary}
[34] \cite{millward1975skeletal}
[35] \cite{bonjour2005dietary}
[36] \cite{phillips2011dietary}
[37] \cite{olaniyan2021dietary}
[38] \cite{kingsley2016acute}
[39] \cite{peake2017muscle}
[40] \cite{pedersen1998recovery}
[41] \cite{wilcock2006water}
[42] \cite{smolak2005sociocultural}
[43] \cite{damas2016resistance}
[44] \cite{macdougall1995time}
[45] \cite{dreyer2010resistance}
[46] \cite{kumar2009age}
[47] \cite{phillips1999resistance}
[48] \cite{schulte2001effects}
[49] \cite{yarasheski1993acute}
[50] \cite{gasier2011cumulative}
[51] \cite{holwerda2018daily}
[52] \cite{tang2008resistance}
[53] \cite{ferrando1997resistance}
[54] \cite{burd2010low}
[55] \cite{welle1995myofibrillar}
[56] \cite{phillips1997mixed}
[57] \cite{mitchell2014acute}
[58] \cite{mayhew2009translational}
[59] \cite{witard2009resistance}
[60] \cite{hasten2000resistance}
[61] \cite{burd2010resistance}
[62] \cite{dreyer2006resistance}
[63] \cite{burd2012muscle}
[64] \cite{wilkinson2008differential}
[65] \cite{kim2005fasted}
[66] \cite{chesley1992changes}
[67] \cite{yarasheski1999resistance}
[68] \cite{fujita2007blood}
[69] \cite{yarasheski1995effect}
[70] \cite{burd2011enhanced}
[71] \cite{fry2013skeletal}
[72] \cite{bell2015day}
[73] \cite{hulston2018resistance}
[74] \cite{drummond2008skeletal}
[75] \cite{mitchell2013muscular}
[76] \cite{mckendry2016short}
[77] \cite{macnaughton2016response}
[78] \cite{witard2012myofibrillar}
[79] \cite{moore2009ingested}
[80] \cite{schoenfeld2018how}
[81] \cite{areta2014reduced}
[82] \cite{areta2013timing}
[83] \cite{west2011rapid}
[84] \cite{esmarck2001timing}
[85] \cite{churchward2020dose}
[86] \cite{dideriksen2011stimulation}
[87] \cite{tipton2007stimulation}
[88] \cite{churchward2012supplementation}
[89] \cite{english2010protecting}
[90] \cite{yang2012myofibrillar}
[91] \cite{willoughby2007effects}
[92] \cite{moore2009differential}
[93] \cite{oikawa2018randomized}
[94] \cite{andersen2005effect}
[95] \cite{borsheim2002essential}
[96] \cite{tang2007minimal}
[97] \cite{howarth2009coingestion}
[98] \cite{tang2009ingestion}
[99] \cite{fujita2009essential}
[100] \cite{pasiakos2013effects}
[101] \cite{roth2021high}
[102] \cite{koopman2006co}
[103] \cite{pennings2011exercising}
[104] \cite{mitchell2015consumption}
[105] \cite{rahbek2014effects}
[106] \cite{beelen2008coingestion}
[107] \cite{bulow2023effect}
[108] \cite{symons2009moderate}
[109] \cite{smith2018effect}
[110] \cite{luiking2014postprandial}
[111] \cite{kanda2013post}
[112] \cite{ormsbee2022pre}
[113] \cite{reis2021effects}
[114] \cite{ramos2021effects}
[115] \cite{snijders2015protein}
[116] \cite{morrison2022sleep}
[117] \cite{betts2011endocrine}
[118] \cite{saracino2020effects}
[119] \cite{kouw2017protein}
[120] \cite{lamon2021effect}
[121] \cite{saner2021exercise}
[122] \cite{holwerda2016physical}
[123] \cite{res2012protein}
[124] \cite{groen2012intragastric}
[125] \cite{holwerda2018protein}
[126] \cite{smeuninx2021effect}
[127] \cite{drummond2012bed}
[128] \cite{monico2013resistance}
[129] \cite{ferrando1996prolonged}
[130] \cite{lyons2023sleep}
[131] \cite{stich2022potential}
[132] \cite{chennaoui2021how}
[133] \cite{buchmann2016sleep}
[134] \cite{kortebein2007effect}
[135] \cite{peake2019recovery}
[136] \cite{reidy2017neuromuscular}
[137] \cite{viana2012effects}
[138] \cite{alley2015effects}
[139] \cite{shioda2019effect}
[140] \cite{miller2020moderate}
[141] \cite{yang2012exercise}
[142] \cite{chennaoui2015sleep}
[143] \cite{madzima2018influence}

